Stable Estimation of Rigid Body Motion using Geometric Mechanics

In this work, asymptotically stable state estimation schemes are proposed for rigid body motion, using the framework of geometric mechanics. Rigorous stability analyses of the estimation schemes presented here guarantee the nonlinear stability of these schemes. The stability of these schemes does not depend on the characteristics of the sensor measurement noise or external disturbances. In addition, they are robust to initial errors in the state estimates and do not need to be re-tuned when sensor noise properties change. In the first part of this dissertation, estimation of rigid body states is considered, given the dynamics model of the rigid body. In the second part, an estimation scheme that does not require knowledge of the dynamics of the rigid body is derived, based on onboard sensor measurements obtained at an appropriate frequency. The frequency of such measurements must be suitably high to resolve the motion of the rigid body. These attitude and pose estimation schemes are obtained by applying the Lagrange-d'Alembert principle from variational mechanics, to a Lagrangian constructed from state estimation errors and a dissipative term linear in the velocity estimation errors.

==> Publications.tex <==

\section*{Publications at New Mexico State University}




\section*{Journal Papers}
\begin{enumerate}
\item {Izadi,~M., \& Sanyal,~A.~K. (2014).
\newblock Rigid body attitude estimation based on the {L}agrange-d'{A}lembert
  principle.
\newblock {\em Automatica}, 50(10), 2570--2577.}

\item {Izadi,~M., \& Sanyal,~A.~K. (2015).
\newblock Rigid body pose estimation based on the {L}agrange-d'{A}lembert principle.
\newblock To appear in {\em Automatica}.}

\item{Br{\'a}s,~S., Izadi,~M., Silvestre,~C., Sanyal,~A., \& Oliveira,~P. (2015).
\newblock Nonlinear Observer for 3{D} Rigid Body Motion Estimation Using Doppler Measurements. \newblock To appear in \emph{IEEE Transactions on Automatic Control.}}

\item {Misra,~G., Izadi,~M., Sanyal,~A.~K., \& Scheeres,~D.~J. (2015).
\newblock Coupled orbit-attitude dynamics and relative state estimation of
  spacecraft near small Solar System bodies.
\newblock To appear in {\em Advances in Space Research}.}

\item {Izadi,~M., Sanyal,~A., Silvestre,~C., \& Oliveira,~P. (2015).
\newblock The Variational Attitude Estimator in the Presence of Bias in Angular Velocity Measurements. \newblock Under preparation.}

\item{Viswanathan,~S.~P., Sanyal,~A.~K., \& Izadi,~M. (2015).
\newblock Smartphone-Based Spacecraft Attitude Determination and Control
System (ADCS) using Internal Momentum Exchange Actuators. \newblock Under preparation.}
\end{enumerate}








\section*{Conference Papers}
\begin{enumerate}
\item{Izadi,~M., Bohn,~J., Lee,~D., Sanyal,~A., Butcher,~E., \& Scheeres,~D. (2013).
\newblock A Nonlinear Observer Design for a Rigid Body in the Proximity of a Spherical Asteroid.
\newblock In {\em Proceedings of the ASME Dynamics Systems and Control Conference}. Palo Alto, CA, USA.}

\item{Br{\'a}s,~S., Izadi,~M., Silvestre,~C., Sanyal,~A., \& Oliveira,~P. (2013).
\newblock Nonlinear Observer for 3D Rigid Body Motion.
\newblock In {\em Proceedings of the $52^{nd}$ IEEE Conference on Decision and Control}. Florence, Italy.}

\item{Sanyal,~A., Izadi,~M., \& Bohn,~J. (2014).
\newblock An Observer for Rigid Body Motion with Almost Global Finite-time Convergence.
\newblock In {\em Proceedings of the ASME Dynamics Systems and Control Conference}. San Antonio, TX, USA.}

\item{Lee,~D., Izadi,~M., Sanyal,~A., Butcher,~E., \& Scheeres,~D. (2014).
\newblock Finite-Time Control for Body-Fixed Hovering of Rigid Spacecraft over an Asteroid.
\newblock In {\em Proceedings of the AAS/AIAA Space Flight Mechanics}. Santa Fe, NM, USA.}

\item {Sanyal,~A.~K., Izadi,~M., \& Butcher,~E.~A. (2014).
\newblock Determination of relative motion of a space object from simultaneous
  measurements of range and range rate.
\newblock In {\em Proceedings of the American Control Conference} (pp. 1607--1612). Portland, OR, USA.}

\item {Sanyal,~A.~K., Izadi,~M., Misra,~G., Samiei,~E., \& Scheeres,~D.~J. (2014).
\newblock Estimation of Dynamics of Space Objects from Visual Feedback During Proximity Operations.
\newblock In {\em Proceedings of the AIAA Space Conference}. San Diego, CA, USA.}

\item {Viswanathan,~S.~P., Sanyal,~A.~K., \& Izadi,~M. (2015).
\newblock Mechatronics Architecture of Smartphone Based Spacecraft ADCS using VSCMG Actuators.
\newblock In {\em Proceedings of the Indian Control Conference}. Chennai, India.}

\item{Izadi,~M., Samiei,~E., Sanyal,~A.~K., \& Kumar,~V. (2015).
\newblock Comparison of an attitude estimator based on the
  {L}agrange-d'{A}lembert principle with some state-of-the-art filters.
\newblock In {\em Proceedings of the IEEE International Conference on Robotics and
  Automation} (pp. 2848--2853). Seattle, WA, USA.}

\item{Samiei,~E., Izadi,~M., Viswanathan,~S.~P., Sanyal,~A.~K., \& Butcher,~E.~A. (2015).
\newblock Robust Stabilization of Rigid Body Attitude Motion in the
  Presence of a Stochastic Input Torque.
\newblock In {\em Proceedings of the IEEE International Conference on Robotics and
  Automation} (pp. 428--433). Seattle, WA, USA.}

\item{Samiei,~E., Izadi,~M., Viswanathan,~S.~P., Sanyal,~A.~K., \& Butcher,~E.~A. (2015).
\newblock Delayed Feedback Asymptotic Stabilization of Rigid Body Attitude Motion
  for Large Rotations.
\newblock In {\em Proceedings of the 12$^{th}$ IFAC Workshop on Time Delay Systems}. Ann Arbor, MI, USA.}

\item{Izadi,~M., Sanyal,~A.~K., Samiei,~E., \& Viswanathan,~S.~P. (2015).
\newblock Discrete-time rigid body attitude state estimation based on the
  discrete {L}agrange-d'{A}lembert principle.
\newblock In {\em Proceedings of the American Control Conference} (pp. 3392--3397). Chicago, IL, USA.}

\item{Izadi,~M., Sanyal,~A.~K., Barany,~E., \& Viswanathan,~S.~P. (2015).
\newblock Rigid Body Motion Estimation based on the Lagrange-d'Alembert Principle.
\newblock In {\em Proceedings of the $54^{nd}$ IEEE Conference on Decision and Control}. Osaka, Japan.}

\item{Izadi,~M., Sanyal,~A.~K., Beard,~R.~W., \& Bai,~H. (2015).
\newblock GPS-Denied Relative Motion Estimation for Fixed-Wing UAV using the Variational Pose Estimator.
\newblock In {\em Proceedings of the $54^{nd}$ IEEE Conference on Decision and Control}. Osaka, Japan.}

\item{Izadi,~M., Sanyal,~A.~K., Silvestre,~C., \& Oliveira,~P. (2016).
\newblock The Variational Attitude Estimator in the Presence of Bias in Angular Velocity Measurements.
\newblock Submitted to {\em the American Control Conference}. Boston, MA, USA.}

\end{enumerate}









%\renewcommand{\bibname}{Conference Papers}
%\begin{thebibliography}{1}
%\nocite{*}
%\bibitem[Nazari et~al.(Jan. 29--Feb. 2, 2012)Nazari, Samiei, Butcher, and
%  Schaub]{Morad}
%M.~Nazari, E.~Samiei, E.A. Butcher, and H.~Schaub.
%\newblock Attitude {S}tabilization {U}sing {N}onlinear {D}elayed{A}ctuator
%  {C}ontrol with an {I}nverse {D}ynamics{A}pproach.
%\newblock \emph{AAS/AIAA Spaceflight Mechanics Meeting, Charleston, SC,Paper
% No. 12-237}, Jan. 29--Feb. 2, 2012.
%
%\bibitem[Samiei et~al.(2012)Samiei, Nazari, Butcher, and Schaub]{Samiei1}
%E.~Samiei, M.~Nazari, E.A. Butcher, and H.~Schaub.
%\newblock Delayed feedback attitude control using neural networks and
%  lyapunov-krasovskii functionals.
%\newblock \emph{AAS/AIAA Spaceflight Mechanics Meeting, Charleston, SC}, 2012.
%  \end{thebibliography}
%
%
%\renewcommand{\bibname}{Journal Papers}
%\begin{thebibliography}{1}
%\bibitem[Samiei et~al.(2013)Samiei, Torkamani, and Butcher]{Samiei}
%Ehsan Samiei, Shahab Torkamani, and Eric~A Butcher.
%\newblock On lyapunov stability of scalar stochastic time-delayed systems.
%\newblock \emph{International Journal of Dynamics and Control}, 1\penalty0
%  (1):\penalty0 64--80, 2013.
%\end{thebibliography}
%
